Who Increases Emergency Department Use? New Insights from the Oregon Health Insurance Experiment

We provide new insights regarding the headline result that Medicaid increased emergency department (ED) use from the Oregon experiment. We find meaningful heterogeneous impacts of Medicaid on ED use using causal machine learning methods. The individualized treatment effect distribution includes a wide range of negative and positive values, suggesting the average effect masks substantial heterogeneity. A small group-about 14% of participants-in the right tail of the distribution drives the overall effect. We identify priority groups with economically significant increases in ED usage based on demographics and previous utilization. Intensive margin effects are an important driver of increases in ED utilization.

==> Tables/Tables_final/itt/t-comp-lr-lp.tex <==
\begin{table}
\caption{\label{tab:comp.rule}Individuals selected by the lottery and the optimal treatment assignment based on integer programming}
\centering
\fontsize{9}{11}\selectfont
\makebox[\textwidth][c]{
\begin{threeparttable}
\begin{tabular}[t]{lrrr}
\toprule
Variable & Not selected & Lottery selected & Difference\\
\midrule
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{Lottery list and baseline characteristics}}\\
\hspace{1em}Age (years)                                          & 39.66   & 39.50   & -0.16      \\
\hspace{1em}Gave phone number                                    & 0.87    & 0.88    & 0.01**     \\
\hspace{1em}English as preferred language                        & 0.88    & 0.85    & -0.03***   \\
\hspace{1em}Female                                               & 0.55    & 0.54    & -0.02***   \\
\hspace{1em}Week of lottery sign up                              & 1.60    & 1.55    & -0.05**    \\
\hspace{1em}Provided P.O. box address                            & 0.03    & 0.03    & -0.00      \\
\hspace{1em}Signed up self for lottery                           & 0.93    & 0.85    & -0.08***   \\
\hspace{1em}Pre-lottery SNAP recipient                           & 0.54    & 0.53    & -0.01      \\
\hspace{1em}Pre-lottery SNAP benefit amount (\textbackslash{}\$) & 1302.79 & 1377.42 & 74.62***   \\
\hspace{1em}Pre-lottery TANF recipient                           & 0.02    & 0.02    & 0.00       \\
\hspace{1em}Pre-lottery TANF benefit amount (\textbackslash{}\$) & 93.60   & 100.17  & 6.58       \\
\hspace{1em}Number of overall visits                             & 0.80    & 0.73    & -0.07***   \\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{Pre-randomization ED use}}                                             \\
\hspace{1em}Number of inpatient visits                           & 0.09    & 0.08    & -0.02***   \\
\hspace{1em}Number of outpatient visits                          & 0.71    & 0.65    & -0.06**    \\
\hspace{1em}Number of on-hours visits                            & 0.47    & 0.42    & -0.05***   \\
\hspace{1em}Number of off-hours visits                           & 0.34    & 0.31    & -0.03**    \\
\hspace{1em}Number of emergent, non-preventable visits           & 0.16    & 0.15    & -0.01*     \\
\hspace{1em}Number of emergent, preventable visits               & 0.06    & 0.06    & -0.01**    \\
\hspace{1em}Number of primary care treatable visits              & 0.27    & 0.26    & -0.01      \\
\hspace{1em}Number of non-emergent visits                        & 0.17    & 0.15    & -0.02**    \\
\hspace{1em}Number ambulatory-care-sensitive visits              & 0.05    & 0.05    & -0.01*     \\
\hspace{1em}Number of visits (chronic conditions)                & 0.15    & 0.12    & -0.03***   \\
\hspace{1em}Number of visits (injury)                            & 0.17    & 0.17    & -0.00      \\
\hspace{1em}Number of visits (skin conditions)                   & 0.05    & 0.04    & -0.00      \\
\hspace{1em}Number of visits (abdominal pain)                    & 0.04    & 0.04    & -0.00      \\
\hspace{1em}Number of visits (back pain)                         & 0.03    & 0.03    & 0.00       \\
\hspace{1em}Number of visits (chest pain)                        & 0.02    & 0.02    & -0.00      \\
\hspace{1em}Number of visits (headache)                          & 0.03    & 0.02    & -0.00      \\
\hspace{1em}Number of visits (mood disorders)                    & 0.03    & 0.02    & -0.00      \\
\hspace{1em}Number of visits (psychiatric conditions)            & 0.06    & 0.05    & -0.01**    \\
\hspace{1em}Sum of total ED charges                              & 935.23  & 831.82  & -103.41*** \\
\hspace{1em}Number of overall visits                             & 1.00    & 0.99    & -0.01      \\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{ED use outcomes}}                                                      \\
\hspace{1em}Number of inpatient visits                           & 0.12    & 0.10    & -0.02***   \\
\hspace{1em}Number of outpatient visits                          & 0.88    & 0.89    & 0.01       \\
\hspace{1em}Number of emergent, non-preventable visits           & 0.21    & 0.21    & -0.00      \\
\hspace{1em}Number of emergent, preventable visits               & 0.07    & 0.08    & 0.00       \\
\hspace{1em}Number of primary care treatable visits              & 0.34    & 0.36    & 0.01       \\
\hspace{1em}Number of non-emergent visits                        & 0.20    & 0.21    & 0.01       \\
\addlinespace[0.3em]
\hline
\multicolumn{4}{l}{\textbf{}}\\
N & 9626 & 15020 & 24646\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item \emph{Notes}: This table reports the means of individual characteristics, pre-randomization ED use and post-treatment outcomes for those selected by the lottery and selected by the optimal treatment assignment solution based on the optimal linear program which minimizes non-emergent ed use under the restriction that a similar number of people are treated as within the lottery (restricted to the number of participants selected by the lottery). The sample consists of 24,613 individuals in the \citeasnoun{taubman2014medicaid} sample with non-missing information on pre-lottery emergency department utilization and SNAP/TANF receipt.
\end{tablenotes}
\end{threeparttable}
}
\end{table}


==> Tables/Tables_final/itt/t-comp-lr-pt.tex <==
\begin{table}

\caption{\label{tab:comp.rule}Individuals selected by the lottery and the optimal treatment assignment rule.}
\centering
\fontsize{9}{11}\selectfont
\makebox[\textwidth][c]{
\begin{threeparttable}
\begin{tabular}[t]{lrrr}
\toprule
Variable & Lottery selected & Rule selected & Difference\\
\midrule
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{Lottery list and baseline characteristics}}\\
\hspace{1em}Age (years) & 39.50 & 40.93 & 1.43***\\
\hspace{1em}Gave phone number & 0.88 & 0.85 & -0.03***\\
\hspace{1em}English as preferred language & 0.85 & 0.95 & 0.10***\\
\hspace{1em}Female & 0.54 & 0.52 & -0.02\\
\hspace{1em}Week of lottery sign up & 1.55 & 1.42 & -0.13***\\
\hspace{1em}Provided P.O. box address & 0.03 & 0.02 & -0.01\\
\hspace{1em}Signed up self for lottery & 0.85 & 0.95 & 0.10***\\
\hspace{1em}Pre-lottery SNAP recipient & 0.53 & 0.67 & 0.14***\\
\hspace{1em}Pre-lottery SNAP benefit amount (\textbackslash{}\$) & 1376.53 & 1465.97 & 89.44**\\
\hspace{1em}Pre-lottery TANF recipient & 0.02 & 0.03 & 0.01\\
\hspace{1em}Pre-lottery TANF benefit amount (\textbackslash{}\$) & 100.09 & 88.96 & -11.13\\
\hspace{1em}Number of overall visits & 0.71 & 2.24 & 1.53***\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{Pre-randomization ED use}}\\
\hspace{1em}Number of inpatient visits & 0.08 & 0.64 & 0.56***\\
\hspace{1em}Number of outpatient visits & 0.63 & 1.61 & 0.98***\\
\hspace{1em}Number of on-hours visits & 0.41 & 1.33 & 0.92***\\
\hspace{1em}Number of off-hours visits & 0.30 & 0.93 & 0.63***\\
\hspace{1em}Number of emergent, non-preventable visits & 0.15 & 0.76 & 0.61***\\
\hspace{1em}Number of emergent, preventable visits & 0.05 & 0.26 & 0.21***\\
\hspace{1em}Number of primary care treatable visits & 0.25 & 0.64 & 0.39***\\
\hspace{1em}Number of non-emergent visits & 0.14 & 0.23 & 0.09***\\
\hspace{1em}Number ambulatory-care-sensitive visits & 0.05 & 0.25 & 0.20***\\
\hspace{1em}Number of visits (chronic conditions) & 0.12 & 0.64 & 0.52***\\
\hspace{1em}Number of visits (injury) & 0.17 & 0.52 & 0.35***\\
\hspace{1em}Number of visits (skin conditions) & 0.04 & 0.11 & 0.07***\\
\hspace{1em}Number of visits (abdominal pain) & 0.03 & 0.07 & 0.04***\\
\hspace{1em}Number of visits (back pain) & 0.03 & 0.05 & 0.02**\\
\hspace{1em}Number of visits (chest pain) & 0.02 & 0.11 & 0.09***\\
\hspace{1em}Number of visits (headache) & 0.02 & 0.03 & 0.01\\
\hspace{1em}Number of visits (mood disorders) & 0.02 & 0.16 & 0.14***\\
\hspace{1em}Number of visits (psychiatric conditions) & 0.05 & 0.32 & 0.27***\\
\hspace{1em}Sum of total ED charges & 808.36 & 3225.36 & 2417.00***\\
\hspace{1em}Number of overall visits & 0.98 & 2.01 & 1.03***\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{ED use outcomes}}\\
\hspace{1em}Number of inpatient visits & 0.10 & 0.38 & 0.28***\\
\hspace{1em}Number of outpatient visits & 0.87 & 1.63 & 0.76***\\
\hspace{1em}Number of emergent, non-preventable visits & 0.20 & 0.44 & 0.24***\\
\hspace{1em}Number of emergent, preventable visits & 0.07 & 0.18 & 0.11***\\
\hspace{1em}Number of primary care treatable visits & 0.35 & 0.62 & 0.27***\\
\hspace{1em}Number of non-emergent visits & 0.20 & 0.36 & 0.16***\\
\addlinespace[0.3em]
\hline
\multicolumn{4}{l}{\textbf{}}\\
N & 9607 & 2258 & 11865\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item \emph{Notes}: This table reports the means of individual characteristics, pre-randomization ED use and post-treatment outcomes for those selected by the lottery and selected by the optimal depth-2 treatment assignment rule. The sample consists of 24,613 individuals in the \citeasnoun{taubman2014medicaid} sample with non-missing information on pre-lottery emergency department utilization and SNAP/TANF receipt.
\end{tablenotes}
\end{threeparttable}
}
\end{table}


==> Tables/Tables_final/itt/tcomp-any-visit-alt-itt.tex <==
\begin{table}[H]

\caption{\label{tab:gates.any.itt}Group average treatment effects of winning the lottery on the propensity of ED use}
\centering
\fontsize{9}{11}\selectfont
\makebox[\textwidth][c]{
\begin{threeparttable}
\begin{tabular}[t]{lrrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Panel A: GRF estimates} & \multicolumn{3}{c}{Panel B: Linear estimates} & \multicolumn{1}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
{Group} & {GATE} & {SE} & {$p$-value} & {GATE} & {SE} & {$p$-value} & {\%~N}\\
\midrule
ATE & 0.02 & 0.01 & 0.01 & 0.02 & 0.01 & 0.00 & 100.00\\
Female: & 0.00 & 0.01 & 0.72 & 0.01 & 0.01 & 0.34 & 0.55\\
Male: & 0.03 & 0.01 & 0.00 & 0.03 & 0.01 & 0.00 & 0.45\\
Gave phone number: No & 0.01 & 0.02 & 0.54 & 0.01 & 0.02 & 0.66 & 0.13\\
Gave phone number: Yes & 0.02 & 0.01 & 0.01 & 0.02 & 0.01 & 0.00 & 0.87\\
English as preferred language: No & 0.01 & 0.01 & 0.59 & 0.00 & 0.01 & 0.73 & 0.14\\
English as preferred language: Yes & 0.02 & 0.01 & 0.01 & 0.02 & 0.01 & 0.01 & 0.86\\
First week sign-up: No & 0.01 & 0.01 & 0.06 & 0.02 & 0.01 & 0.01 & 0.62\\
First week sign-up: Yes & 0.02 & 0.01 & 0.06 & 0.01 & 0.01 & 0.16 & 0.38\\
Pre-lottery SNAP recipient: No & 0.00 & 0.01 & 0.94 & 0.00 & 0.01 & 0.62 & 0.46\\
Pre-lottery SNAP recipient: Yes & 0.03 & 0.01 & 0.00 & 0.02 & 0.01 & 0.01 & 0.54\\
Pre-lottery TANF recipient: No & 0.02 & 0.01 & 0.01 & 0.02 & 0.01 & 0.00 & 0.98\\
Pre-lottery TANF recipient: Yes & -0.01 & 0.04 & 0.78 & 0.01 & 0.04 & 0.82 & 0.02\\
Age ≥ 50: No & 0.02 & 0.01 & 0.00 & 0.02 & 0.01 & 0.00 & 0.75\\
Age ≥ 50: Yes & -0.01 & 0.01 & 0.67 & 0.00 & 0.01 & 0.77 & 0.25\\
Two+ household members on lottery list: No & 0.01 & 0.01 & 0.06 & 0.01 & 0.01 & 0.06 & 0.80\\
Two+ household members on lottery list: Yes & 0.03 & 0.01 & 0.02 & 0.04 & 0.01 & 0.00 & 0.20\\
Any pre-lottery ED visit No & 0.01 & 0.01 & 0.07 & 0.02 & 0.01 & 0.02 & 0.69\\
Any pre-lottery ED visit: Yes & 0.02 & 0.01 & 0.05 & 0.02 & 0.01 & 0.09 & 0.31\\
Any pre-lottery on-hours ED visit: No & 0.01 & 0.01 & 0.03 & 0.02 & 0.01 & 0.01 & 0.77\\
Any pre-lottery on-hours ED visit: Yes & 0.02 & 0.01 & 0.11 & 0.02 & 0.01 & 0.13 & 0.23\\
Any pre-lottery off-hours ED visit: No & 0.01 & 0.01 & 0.04 & 0.01 & 0.01 & 0.03 & 0.81\\
Any pre-lottery off-hours ED visit: Yes & 0.02 & 0.01 & 0.08 & 0.02 & 0.01 & 0.16 & 0.19\\
Any pre-lottery emergent, non-preventable ED visit: No & 0.01 & 0.01 & 0.02 & 0.02 & 0.01 & 0.01 & 0.87\\
Any pre-lottery emergent, non-preventable ED visit: Yes & 0.02 & 0.02 & 0.22 & 0.02 & 0.02 & 0.29 & 0.13\\
Any pre-lottery emergent, preventable ED visit: No & 0.02 & 0.01 & 0.01 & 0.02 & 0.01 & 0.00 & 0.92\\
Any pre-lottery emergent, preventable ED visit: Yes & 0.00 & 0.02 & 0.86 & 0.00 & 0.02 & 0.83 & 0.08\\
Any pre-lottery primary care treatable ED visit: No & 0.01 & 0.01 & 0.10 & 0.02 & 0.01 & 0.02 & 0.81\\
Any pre-lottery primary care treatable ED visit: Yes & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.03 & 0.19\\
Any pre-lottery non-emergent ED visit: No & 0.01 & 0.01 & 0.03 & 0.02 & 0.01 & 0.01 & 0.86\\
Any pre-lottery non-emergent ED visit: Yes & 0.03 & 0.02 & 0.06 & 0.02 & 0.02 & 0.17 & 0.14\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item \emph{Notes}: This table reports the group average treatment effects of winning the lottery based on generalized random forests in Panel A and those based on a linear IV subsample analysis approach in Panel B. The first row reproduces the overall average effect. The baseline sample consists of 24,615 individuals in the \citeasnoun{taubman2014medicaid} sample with non-missing information on pre-lottery emergency department utilization and SNAP/TANF receipt.
\end{tablenotes}
\end{threeparttable}
}
\end{table}

% old, simple def
% Any pre-lottery emergent, non-preventable ED visit: No & 0.01 & 0.01 & 0.07 & 0.01 & 0.01 & 0.03 & 0.79\\
% Any pre-lottery emergent, non-preventable ED visit: Yes & 0.03 & 0.01 & 0.02 & 0.03 & 0.01 & 0.07 & 0.21\\
% Any pre-lottery emergent, preventable ED visit: No & 0.01 & 0.01 & 0.02 & 0.02 & 0.01 & 0.00 & 0.90\\
% Any pre-lottery emergent, preventable ED visit: Yes & 0.03 & 0.02 & 0.15 & 0.03 & 0.02 & 0.13 & 0.10\\
% Any pre-lottery primary care treatable ED visit: No & 0.01 & 0.01 & 0.10 & 0.01 & 0.01 & 0.03 & 0.74\\
% Any pre-lottery primary care treatable ED visit: Yes & 0.03 & 0.01 & 0.02 & 0.03 & 0.01 & 0.05 & 0.26\\
% Any pre-lottery non-emergent ED visit: No & 0.01 & 0.01 & 0.04 & 0.02 & 0.01 & 0.01 & 0.86\\
% Any pre-lottery non-emergent ED visit: Yes & 0.03 & 0.02 & 0.07 & 0.02 & 0.02 & 0.18 & 0.14\\


==> Tables/Tables_final/itt/tdescriptives-itt.tex <==
\begin{table}[h]

\caption{\label{tab:desc.base.itt}Descriptive Statistics}
\centering
\fontsize{9}{11}\selectfont
\begin{threeparttable}
\begin{tabular}[t]{lrrrrr}
\toprule
Variable & Mean & SD & Median & Min & Max\\
\midrule
\addlinespace[0.3em]
\multicolumn{6}{l}{\textbf{Lottery list and baseline characteristics}}\\
\hspace{1em}Age (years) & 39.60 & 12.05 & 39.0 & 20 & 63\\
\hspace{1em}Gave phone number & 0.87 & 0.34 & 1.0 & 0 & 1\\
\hspace{1em}English as preferred language & 0.86 & 0.34 & 1.0 & 0 & 1\\
\hspace{1em}Female & 0.55 & 0.50 & 1.0 & 0 & 1\\
\hspace{1em}Week of lottery sign up & 1.58 & 1.62 & 1.0 & 0 & 5\\
\hspace{1em}Provided P.O. box address & 0.03 & 0.16 & 0.0 & 0 & 1\\
\hspace{1em}Signed up self for lottery & 0.90 & 0.30 & 1.0 & 0 & 1\\
\hspace{1em}Pre-lottery SNAP recipient & 0.54 & 0.50 & 1.0 & 0 & 1\\
\hspace{1em}Pre-lottery SNAP benefit amount (\$) & 1331.94 & 1863.76 & 522.5 & 0 & 20745\\
\hspace{1em}Pre-lottery TANF recipient & 0.02 & 0.15 & 0.0 & 0 & 1\\
\hspace{1em}Pre-lottery TANF benefit amount (\$) & 96.16 & 694.70 & 0.0 & 0 & 16031\\
\hspace{1em}Number of overall visits & 0.77 & 1.86 & 0.0 & 0 & 17\\
\addlinespace[0.3em]
\multicolumn{6}{l}{\textbf{Pre-randomization ED use}}\\
\hspace{1em}Number of inpatient visits & 0.09 & 0.41 & 0.0 & 0 & 6\\
\hspace{1em}Number of outpatient visits & 0.69 & 1.71 & 0.0 & 0 & 16\\
\hspace{1em}Number of on-hours visits & 0.45 & 1.23 & 0.0 & 0 & 13\\
\hspace{1em}Number of off-hours visits & 0.33 & 0.92 & 0.0 & 0 & 10\\
\hspace{1em}Number of emergent, non-preventable visits & 0.16 & 0.50 & 0.0 & 0 & 9\\
\hspace{1em}Number of emergent, preventable visits & 0.06 & 0.28 & 0.0 & 0 & 6\\
\hspace{1em}Number of primary care treatable visits & 0.27 & 0.75 & 0.0 & 0 & 12\\
\hspace{1em}Number of non-emergent visits & 0.16 & 0.58 & 0.0 & 0 & 12\\
\hspace{1em}Number ambulatory-care-sensitive visits & 0.05 & 0.30 & 0.0 & 0 & 5\\
\hspace{1em}Number of visits (chronic conditions) & 0.14 & 0.64 & 0.0 & 0 & 9\\
\hspace{1em}Number of visits (injury) & 0.17 & 0.56 & 0.0 & 0 & 6\\
\hspace{1em}Number of visits (skin conditions) & 0.05 & 0.31 & 0.0 & 0 & 5\\
\hspace{1em}Number of visits (abdominal pain) & 0.04 & 0.27 & 0.0 & 0 & 5\\
\hspace{1em}Number of visits (back pain) & 0.03 & 0.26 & 0.0 & 0 & 5\\
\hspace{1em}Number of visits (chest pain) & 0.02 & 0.18 & 0.0 & 0 & 3\\
\hspace{1em}Number of visits (headache) & 0.02 & 0.23 & 0.0 & 0 & 4\\
\hspace{1em}Number of visits (mood disorders) & 0.02 & 0.23 & 0.0 & 0 & 5\\
\hspace{1em}Number of visits (psychiatric conditions) & 0.06 & 0.38 & 0.0 & 0 & 6\\
\hspace{1em}Sum of total ED charges & 894.85 & 2593.46 & 0.0 & 0 & 42315\\
\hspace{1em}Any overall visit & 0.34 & 0.47 & 0.0 & 0 & 1\\
\addlinespace[0.3em]
\multicolumn{6}{l}{\textbf{ED use outcomes}}\\
\hspace{1em}Any inpatient visit & 0.07 & 0.26 & 0.0 & 0 & 1\\
\hspace{1em}Any outpatient visit & 0.32 & 0.47 & 0.0 & 0 & 1\\
\hspace{1em}Any emergent, non-preventable visit & 0.16 & 0.37 & 0.0 & 0 & 1\\
\hspace{1em}Any emergent, preventable visit & 0.10 & 0.30 & 0.0 & 0 & 1\\
\hspace{1em}Any primary care treatable visit & 0.22 & 0.41 & 0.0 & 0 & 1\\
\hspace{1em}Any non-emergent visit & 0.16 & 0.37 & 0.0 & 0 & 1\\
\hspace{1em}Number of overall visits & 1.00 & 2.41 & 0.0 & 0 & 22\\
\hspace{1em}Number of inpatient visits & 0.11 & 0.53 & 0.0 & 0 & 7\\
\hspace{1em}Number of outpatient visits & 0.89 & 2.21 & 0.0 & 0 & 21\\
\hspace{1em}Number of emergent, non-preventable visits & 0.21 & 0.69 & 0.0 & 0 & 14\\
\hspace{1em}Number of emergent, preventable visits & 0.07 & 0.35 & 0.0 & 0 & 8\\
\hspace{1em}Number of primary care treatable visits & 0.35 & 0.96 & 0.0 & 0 & 16\\
\hspace{1em}Number of non-emergent visits & 0.20 & 0.70 & 0.0 & 0 & 13\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item \emph{Notes}: This table presents descriptive statistics based on the Oregon Health Insurance Experiment data. The sample consists of 24,615 individuals in the \citet{taubman2014medicaid} sample with non-missing information on pre-lottery emergency department utilization and SNAP/TANF receipt. The pre-randomization SNAP and TANF benefits are total household benefits received from January 2007 through the individual's lottery notification date. The pre-randomization ED use measures are with respect to utilization between January 1, 2007 and March 9, 2008.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/Tables_final/itt/tmain-ext-itt.tex <==

\begin{landscape}\begin{table}[!htb]

\caption{\label{tab:main.ext.itt}Treatment effect estimates of winning the lottery on ED use}
\centering
\fontsize{8}{10}\selectfont
\makebox[\textwidth][c]{
\begin{threeparttable}
\begin{tabular}[t]{lrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{GRF estimates} & \multicolumn{3}{c}{Linear estimates} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
{Variable} & {ATE} & {SE} & {$p$-value} & {ATE} & {SE} & {$p$-value}\\
\midrule
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{Extensive margin}}\\
\hspace{1em}Any overall visit & 0.032 & 0.013 & 0.010 & 0.017 & 0.006 & 0.004\\
\hspace{1em}Any inpatient visit & -0.003 & 0.007 & 0.594 & -0.003 & 0.003 & 0.424\\
\hspace{1em}Any outpatient visit & 0.039 & 0.012 & 0.001 & 0.020 & 0.006 & 0.001\\
\hspace{1em}Any emergent, non-preventable visit & 0.008 & 0.009 & 0.379 & 0.002 & 0.005 & 0.731\\
\hspace{1em}Any emergent, preventable visit & -0.001 & 0.008 & 0.857 & 0.010 & 0.004 & 0.010\\
\hspace{1em}Any primary care treatable visit & 0.029 & 0.011 & 0.007 & 0.017 & 0.005 & 0.001\\
\hspace{1em}Any non-emergent visit & 0.036 & 0.009 & 0.000 & 0.016 & 0.005 & 0.001\\
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{Intensive margin}}\\
\hspace{1em}Number of overall visits & 0.141 & 0.045 & 0.002 & 0.093 & 0.026 & 0.000\\
\hspace{1em}Number of inpatient visits & -0.003 & 0.011 & 0.799 & -0.004 & 0.006 & 0.516\\
\hspace{1em}Number of outpatient visits & 0.142 & 0.042 & 0.001 & 0.096 & 0.024 & 0.000\\
\hspace{1em}Number of emergent, non-preventable visits & 0.034 & 0.014 & 0.016 & 0.010 & 0.008 & 0.224\\
\hspace{1em}Number of emergent, preventable visits & 0.000 & 0.008 & 0.954 & 0.009 & 0.004 & 0.034\\
\hspace{1em}Number of primary care treatable visits & 0.064 & 0.019 & 0.001 & 0.042 & 0.011 & 0.000\\
\hspace{1em}Number of non-emergent visits & 0.045 & 0.014 & 0.002 & 0.026 & 0.008 & 0.002\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item Note: Estimates for the ATE and quantiles of the ITE using the Oregon Health Insurance Experiment data.
\end{tablenotes}
\end{threeparttable}
}
\end{table}
\end{landscape}

% old, simple def
% \hspace{1em}Any emergent, non-preventable visit & 0.008 & 0.009 & 0.379 & 0.001 & 0.005 & 0.870\\
% \hspace{1em}Any emergent, preventable visit & -0.001 & 0.008 & 0.857 & 0.009 & 0.004 & 0.022\\
% \hspace{1em}Any primary care treatable visit & 0.029 & 0.011 & 0.007 & 0.016 & 0.005 & 0.002\\
% \hspace{1em}Any non-emergent visit & 0.036 & 0.009 & 0.000 & 0.017 & 0.005 & 0.000\\


==> Tables/Tables_final/itt/tqte-ext-itt.tex <==
\begin{table}[t]

\caption{\label{tab:qte.ext.itt}Quantile treatment effect estimates of winning the lottery on ED use}
\centering
\fontsize{8}{10}\selectfont
\begin{threeparttable}
\begin{tabular}[t]{lrrrrrr}
\toprule
{Variable} & {ATE} & {Minimum} & {25\%} & {50\%} & {75\%} & {Max}\\
\midrule
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{Extensive margin}}\\
\hspace{1em}Any overall visit & 0.032 & -0.049 & 0.016 & 0.031 & 0.048 & 0.125\\
\hspace{1em}Any inpatient visit & -0.003 & -0.052 & -0.008 & -0.002 & 0.003 & 0.036\\
\hspace{1em}Any outpatient visit & 0.039 & -0.035 & 0.023 & 0.040 & 0.056 & 0.123\\
\hspace{1em}Any emergent, non-preventable visit & 0.008 & -0.060 & -0.005 & 0.008 & 0.021 & 0.081\\
\hspace{1em}Any emergent, preventable visit & -0.001 & -0.070 & -0.006 & 0.002 & 0.008 & 0.044\\
\hspace{1em}Any primary care treatable visit & 0.029 & -0.021 & 0.016 & 0.027 & 0.041 & 0.099\\
\hspace{1em}Any non-emergent visit & 0.036 & -0.002 & 0.023 & 0.032 & 0.044 & 0.111\\
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{Intensive margin}}\\
\hspace{1em}Number of overall visits & 0.141 & -0.044 & 0.058 & 0.095 & 0.156 & 1.546\\
\hspace{1em}Number of inpatient visits & -0.003 & -0.076 & -0.011 & -0.002 & 0.005 & 0.139\\
\hspace{1em}Number of outpatient visits & 0.142 & -0.047 & 0.061 & 0.097 & 0.153 & 1.548\\
\hspace{1em}Number of emergent, non-preventable visits & 0.034 & -0.027 & 0.009 & 0.022 & 0.041 & 0.391\\
\hspace{1em}Number of emergent, preventable visits & 0.000 & -0.037 & -0.007 & -0.001 & 0.004 & 0.129\\
\hspace{1em}Number of primary care treatable visits & 0.064 & -0.023 & 0.027 & 0.042 & 0.069 & 0.639\\
\hspace{1em}Number of non-emergent visits & 0.045 & -0.009 & 0.023 & 0.032 & 0.051 & 0.404\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item Note: Estimates for quantiles of the ITE using the Oregon Health Insurance Experiment data.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/Tables_final/itt/trule-comp.tex <==
\begin{table}

\caption{\label{tab:comp.rule}Individuals selected by the lottery and the optimal treatment assignment rule.}
\centering
\fontsize{9}{11}\selectfont
\makebox[\textwidth][c]{
\begin{threeparttable}
\begin{tabular}[t]{lrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Panel A: Full sample} & \multicolumn{3}{c}{Panel B: Subsample with $p<0.1$} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
Variable & Lottery selected & Rule selected & Difference\\
\midrule
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{Lottery list and baseline characteristics}}\\
\hspace{1em}Age (years) & 39.50 & 40.93 & 1.43***\\
\hspace{1em}Gave phone number & 0.88 & 0.85 & -0.03***\\
\hspace{1em}English as preferred language & 0.85 & 0.95 & 0.10***\\
\hspace{1em}Female & 0.54 & 0.52 & -0.02*\\
\hspace{1em}Week of lottery sign up & 1.55 & 1.42 & -0.13***\\
\hspace{1em}Provided P.O. box address & 0.03 & 0.02 & -0.01***\\
\hspace{1em}Signed up self for lottery & 0.85 & 0.95 & 0.10***\\
\hspace{1em}ZIP code from MSA & 1.00 & 1.00 & 0.00\\
\hspace{1em}Pre-lottery SNAP recipient & 0.53 & 0.67 & 0.14***\\
\hspace{1em}Pre-lottery SNAP benefit amount (\textbackslash{}\$) & 1376.53 & 1465.97 & 89.44**\\
\hspace{1em}Pre-lottery TANF recipient & 0.02 & 0.03 & 0.01**\\
\hspace{1em}Pre-lottery TANF benefit amount (\textbackslash{}\$) & 100.09 & 88.96 & -11.13\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{Pre-randomization ED use}}\\
\hspace{1em}Number of overall visits & 0.71 & 2.24 & 1.53***\\
\hspace{1em}Number of inpatient visits & 0.08 & 0.64 & 0.56***\\
\hspace{1em}Number of outpatient visits & 0.63 & 1.61 & 0.98***\\
\hspace{1em}Number of on-hours visits & 0.41 & 1.33 & 0.92***\\
\hspace{1em}Number of off-hours visits & 0.30 & 0.93 & 0.63***\\
\hspace{1em}Number of emergent, non-preventable visits & 0.15 & 0.76 & 0.61***\\
\hspace{1em}Number of emergent, preventable visits & 0.05 & 0.26 & 0.21***\\
\hspace{1em}Number of primary care treatable visits & 0.25 & 0.64 & 0.39***\\
\hspace{1em}Number of non-emergent visits & 0.14 & 0.23 & 0.09***\\
\hspace{1em}Number ambulatory-care-sensitive visits & 0.05 & 0.25 & 0.20***\\
\hspace{1em}Number of visits (chronic conditions) & 0.12 & 0.64 & 0.52***\\
\hspace{1em}Number of visits (injury) & 0.17 & 0.52 & 0.35***\\
\hspace{1em}Number of visits (skin conditions) & 0.04 & 0.11 & 0.07***\\
\hspace{1em}Number of visits (abdominal pain) & 0.03 & 0.07 & 0.04***\\
\hspace{1em}Number of visits (back pain) & 0.03 & 0.05 & 0.02***\\
\hspace{1em}Number of visits (chest pain) & 0.02 & 0.11 & 0.09***\\
\hspace{1em}Number of visits (headache) & 0.02 & 0.03 & 0.01**\\
\hspace{1em}Number of visits (mood disorders) & 0.02 & 0.16 & 0.14***\\
\hspace{1em}Number of visits (psychiatric conditions) & 0.05 & 0.32 & 0.27***\\
\hspace{1em}Sum of total ED charges & 808.36 & 3225.36 & 2417.00***\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{ED use outcomes}}\\
\hspace{1em}Number of overall visits & 0.98 & 2.01 & 1.03***\\
\hspace{1em}Number of inpatient visits & 0.10 & 0.38 & 0.28***\\
\hspace{1em}Number of outpatient visits & 0.87 & 1.63 & 0.76***\\
\hspace{1em}Number of emergent, non-preventable visits & 0.20 & 0.44 & 0.24***\\
\hspace{1em}Number of emergent, preventable visits & 0.07 & 0.18 & 0.11***\\
\hspace{1em}Number of primary care treatable visits & 0.35 & 0.62 & 0.27***\\
\hspace{1em}Number of non-emergent visits & 0.20 & 0.36 & 0.16***\\
\addlinespace[0.3em]
\hline
\multicolumn{4}{l}{\textbf{}}\\
N & 9607 & 2258 & 11865\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item \emph{Notes}: This table reports the means of individual characteristics, pre-randomization ED use and post-treatment outcomes for those selected by the lottery and selected by the optimal depth-2 treatment assignment rule. The sample consists of 24,613 individuals in the \citeasnoun{taubman2014medicaid} sample with non-missing information on pre-lottery emergency department utilization and SNAP/TANF receipt.
\end{tablenotes}
\end{threeparttable}
}
\end{table}


==> Tables/Tables_final/itt/tvarimp-all-itt.tex <==
\begin{table}[t]

\caption{\label{tab:varimp.all}Variable importance scores}
\centering
\fontsize{8}{10}\selectfont
\makebox[\textwidth][c]{
\begin{threeparttable}
\begin{tabular}[t]{lr}
\toprule
Variable & Importance\\
\midrule
\addlinespace[0.3em]
\multicolumn{2}{c}{\textbf{Any visit}}\\
\hspace{1em}Pre-lottery SNAP benefit amount (\$) & 0.23\\
\hspace{1em}Age (years) & 0.16\\
\hspace{1em}Sum of total ED charges & 0.09\\
\hspace{1em}Number of emergent, non-preventable visits & 0.08\\
\hspace{1em}Number of primary care treatable visits & 0.08\\
\hspace{1em}Female & 0.04\\
\hspace{1em}Number of non-emergent visits & 0.04\\
\hspace{1em}Week of lottery sign up & 0.04\\
\hspace{1em}Pre-lottery SNAP recipient & 0.02\\
\hspace{1em}Number of emergent, preventable visits & 0.02\\
\addlinespace[0.3em]
\multicolumn{2}{c}{\textbf{Any non-emergent visit}}\\
\hspace{1em}Sum of total ED charges & 0.14\\
\hspace{1em}Number of primary care treatable visits & \vphantom{1} 0.13\\
\hspace{1em}Number of outpatient visits & 0.12\\
\hspace{1em}Pre-lottery SNAP benefit amount (\$) & 0.11\\
\hspace{1em}Number of non-emergent visits & \vphantom{1} 0.08\\
\hspace{1em}Age (years) & 0.08\\
\hspace{1em}Number of emergent, non-preventable visits & 0.07\\
\hspace{1em}Number of emergent, preventable visits & 0.04\\
\hspace{1em}Number of inpatient visits & 0.04\\
\hspace{1em}Number of visits (chronic conditions) & 0.02\\
\addlinespace[0.3em]
\multicolumn{2}{c}{\textbf{Number of visits}}\\
\hspace{1em}Number of primary care treatable visits & 0.13\\
\hspace{1em}Sum of total ED charges & 0.13\\
\hspace{1em}Number of emergent, non-preventable visits & 0.11\\
\hspace{1em}Number of outpatient visits & \vphantom{1} 0.09\\
\hspace{1em}Number of overall visits & 0.08\\
\hspace{1em}Number of non-emergent visits & 0.08\\
\hspace{1em}Number of emergent, preventable visits & 0.06\\
\hspace{1em}Number of off-hours visits & \vphantom{1} 0.06\\
\hspace{1em}Pre-lottery SNAP benefit amount (\$) & 0.06\\
\hspace{1em}Age (years) & 0.03\\
\addlinespace[0.3em]
\multicolumn{2}{c}{\textbf{Number of non-emergent visits}}\\
\hspace{1em}Number of emergent, non-preventable visits & 0.17\\
\hspace{1em}Number of primary care treatable visits & 0.16\\
\hspace{1em}Sum of total ED charges & 0.12\\
\hspace{1em}Number of non-emergent visits & 0.10\\
\hspace{1em}Number of outpatient visits & 0.09\\
\hspace{1em}Number of overall visits & 0.06\\
\hspace{1em}Number of off-hours visits & 0.06\\
\hspace{1em}Number of emergent, preventable visits & 0.05\\
\hspace{1em}Pre-lottery SNAP benefit amount (\$) & 0.04\\
\hspace{1em}Number of inpatient visits & 0.03\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item Note: 
\end{tablenotes}
\end{threeparttable}
}
\end{table}


==> Tables/Tables_final/itt/tvarimp-any-itt.tex <==
\begin{table}[t]

\caption{\label{tab:varimp.any}Variable importance scores}
\centering
\fontsize{8}{10}\selectfont
\makebox[\textwidth][c]{
\begin{threeparttable}
\begin{tabular}[t]{lrlr}
\toprule
\multicolumn{2}{c}{Any visit} & \multicolumn{2}{c}{Any non-emergent visit} \\
\cmidrule(l{3pt}r{3pt}){1-2} \cmidrule(l{3pt}r{3pt}){3-4}
Variable & Importance & Variable & Importance\\
\midrule
Pre-lottery SNAP benefit amount (\$) & 0.23 & Sum of total ED charges & 0.14\\
Age (years) & 0.16 & Number of primary care treatable visits & 0.13\\
Sum of total ED charges & 0.09 & Number of outpatient visits & 0.12\\
Number of emergent, non-preventable visits & 0.08 & Pre-lottery SNAP benefit amount (\$) & 0.11\\
Number of primary care treatable visits & 0.08 & Number of non-emergent visits & 0.08\\
Female & 0.04 & Age (years) & 0.08\\
Number of non-emergent visits & 0.04 & Number of emergent, non-preventable visits & 0.07\\
Week of lottery sign up & 0.04 & Number of emergent, preventable visits & 0.04\\
Pre-lottery SNAP recipient & 0.02 & Number of inpatient visits & 0.04\\
Number of emergent, preventable visits & 0.02 & Number of visits (chronic conditions) & 0.02\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item Note: 
\end{tablenotes}
\end{threeparttable}
}
\end{table}


==> Tables/Tables_final/itt/tvarimp-ne-itt.tex <==
\begin{table}[t]

\caption{\label{tab:varimp.ne}Variable importance scores}
\centering
\fontsize{8}{10}\selectfont
\makebox[\textwidth][c]{
\begin{threeparttable}
\begin{tabular}[t]{lrlr}
\toprule
\multicolumn{2}{c}{Any non-emergent visit} & \multicolumn{2}{c}{Number of nonemergent visits} \\
\cmidrule(l{3pt}r{3pt}){1-2} \cmidrule(l{3pt}r{3pt}){3-4}
Variable & Importance & Variable & Importance\\
\midrule
Sum of total ED charges & 0.14 & Number of emergent, non-preventable visits & 0.17\\
Number of primary care treatable visits & 0.13 & Number of primary care treatable visits & 0.16\\
Number of outpatient visits & 0.12 & Sum of total ED charges & 0.12\\
Pre-lottery SNAP benefit amount (\$) & 0.11 & Number of non-emergent visits & 0.10\\
Number of non-emergent visits & 0.08 & Number of outpatient visits & 0.09\\
Age (years) & 0.08 & Number of overall visits & 0.06\\
Number of emergent, non-preventable visits & 0.07 & Number of off-hours visits & 0.06\\
Number of emergent, preventable visits & 0.04 & Number of emergent, preventable visits & 0.05\\
Number of inpatient visits & 0.04 & Pre-lottery SNAP benefit amount (\$) & 0.04\\
Number of visits (chronic conditions) & 0.02 & Number of inpatient visits & 0.03\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item Note: 
\end{tablenotes}
\end{threeparttable}
}
\end{table}


==> Tables/Tables_final/itt/tvarimp-num-itt.tex <==
\begin{table}[t]

\caption{\label{tab:varimp.num}Variable importance scores}
\centering
\fontsize{8}{10}\selectfont
\makebox[\textwidth][c]{
\begin{threeparttable}
\begin{tabular}[t]{lrlr}
\toprule
\multicolumn{2}{c}{Number of visits} & \multicolumn{2}{c}{Number of nonemergent visits} \\
\cmidrule(l{3pt}r{3pt}){1-2} \cmidrule(l{3pt}r{3pt}){3-4}
Variable & Importance & Variable & Importance\\
\midrule
Number of primary care treatable visits & 0.13 & Number of emergent, non-preventable visits & 0.17\\
Sum of total ED charges & 0.13 & Number of primary care treatable visits & 0.16\\
Number of emergent, non-preventable visits & 0.11 & Sum of total ED charges & 0.12\\
Number of outpatient visits & 0.09 & Number of non-emergent visits & 0.10\\
Number of overall visits & 0.08 & Number of outpatient visits & 0.09\\
Number of non-emergent visits & 0.08 & Number of overall visits & 0.06\\
Number of emergent, preventable visits & 0.06 & Number of off-hours visits & 0.06\\
Number of off-hours visits & 0.06 & Number of emergent, preventable visits & 0.05\\
Pre-lottery SNAP benefit amount (\$) & 0.06 & Pre-lottery SNAP benefit amount (\$) & 0.04\\
Age (years) & 0.03 & Number of inpatient visits & 0.03\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item Note: 
\end{tablenotes}
\end{threeparttable}
}
\end{table}


==> Tables/Tables_final/tmain-ext.tex <==

\begin{landscape}\begin{table}[H]

\caption{\label{tab:main.ext}Treatment effect estimates}
\centering
\fontsize{9}{11}\selectfont
\makebox[\textwidth][c]{
\begin{threeparttable}
\begin{tabular}[t]{lrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{GRF estimates} & \multicolumn{3}{c}{Linear estimates} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
{Variable} & {LATE} & {SE} & {$p$-value} & {LATE} & {SE} & {$p$-value}\\
\midrule
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{Extensive margin}}\\
\hspace{1em}Any overall visit & 0.075 & 0.047 & 0.108 & 0.065 & 0.045 & 0.152\\
\hspace{1em}Any inpatient visit & -0.008 & 0.022 & 0.715 & -0.024 & 0.023 & 0.296\\
\hspace{1em}Any outpatient visit & 0.097 & 0.046 & 0.034 & 0.094 & 0.044 & 0.035\\
\hspace{1em}Any emergent, non-preventable visit & -0.005 & 0.033 & 0.871 & 0.006 & 0.033 & 0.852\\
\hspace{1em}Any emergent, preventable visit & -0.005 & 0.025 & 0.845 & -0.022 & 0.027 & 0.409\\
\hspace{1em}Any primary care treatable visit & 0.078 & 0.038 & 0.041 & 0.073 & 0.038 & 0.057\\
\hspace{1em}Any non-emergent visit & 0.120 & 0.032 & 0.000 & 0.093 & 0.033 & 0.005\\
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{Intensive margin}}\\
\hspace{1em}Number of overall visits & 0.424 & 0.153 & 0.006 & 0.397 & 0.159 & 0.013\\
\hspace{1em}Number of inpatient visits & 0.000 & 0.037 & 0.995 & -0.025 & 0.040 & 0.527\\
\hspace{1em}Number of outpatient visits & 0.424 & 0.146 & 0.004 & 0.413 & 0.146 & 0.005\\
\hspace{1em}Number of emergent, non-preventable visits & 0.099 & 0.048 & 0.040 & 0.090 & 0.048 & 0.063\\
\hspace{1em}Number of emergent, preventable visits & -0.014 & 0.027 & 0.602 & -0.021 & 0.028 & 0.447\\
\hspace{1em}Number of primary care treatable visits & 0.201 & 0.062 & 0.001 & 0.198 & 0.068 & 0.003\\
\hspace{1em}Number of non-emergent visits & 0.144 & 0.048 & 0.003 & 0.136 & 0.048 & 0.005\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item Note: Estimates for the ATE and quantiles of the ITE distribution using the Oregon Health Insurance Experiment data.
\end{tablenotes}
\end{threeparttable}
}
\end{table}
\end{landscape}

% old, simple def
% \hspace{1em}Any emergent, non-preventable visit & -0.005 & 0.033 & 0.871 & 0.000 & 0.033 & 0.996\\
% \hspace{1em}Any emergent, preventable visit & -0.005 & 0.025 & 0.845 & -0.023 & 0.027 & 0.387\\
% \hspace{1em}Any primary care treatable visit & 0.078 & 0.038 & 0.041 & 0.066 & 0.038 & 0.083\\
% \hspace{1em}Any non-emergent visit & 0.120 & 0.032 & 0.000 & 0.089 & 0.033 & 0.008\\


==> Tables/Tables_final/tqte-ext.tex <==
\begin{table}[t]

\caption{\label{tab:qte.ext}Empirical quantiles of the distribution of individualized treatment effects of Medicaid on ED use}
\centering
\fontsize{9}{11}\selectfont
\begin{threeparttable}
\begin{tabular}[t]{lrrrrrr}
\toprule
{Variable} & {LATE} & {Minimum} & {25\%} & {50\%} & {75\%} & {Max}\\
\midrule
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{Extensive margin}}\\
\hspace{1em}Any overall visit & 0.075 & -0.182 & 0.057 & 0.105 & 0.157 & 0.353\\
\hspace{1em}Any inpatient visit & -0.008 & -0.160 & -0.027 & -0.007 & 0.010 & 0.086\\
\hspace{1em}Any outpatient visit & 0.097 & -0.141 & 0.082 & 0.129 & 0.176 & 0.363\\
\hspace{1em}Any emergent, non-preventable visit & -0.005 & -0.244 & -0.017 & 0.027 & 0.060 & 0.186\\
\hspace{1em}Any emergent, preventable visit & -0.005 & -0.260 & -0.018 & 0.006 & 0.026 & 0.116\\
\hspace{1em}Any primary care treatable visit & 0.078 & -0.081 & 0.057 & 0.090 & 0.129 & 0.313\\
\hspace{1em}Any non-emergent visit & 0.120 & -0.002 & 0.084 & 0.111 & 0.141 & 0.323\\
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{Intensive margin}}\\
\hspace{1em}Number of overall visits & 0.424 & -0.191 & 0.206 & 0.318 & 0.468 & 4.824\\
\hspace{1em}Number of inpatient visits & 0.000 & -0.277 & -0.035 & -0.007 & 0.017 & 0.459\\
\hspace{1em}Number of outpatient visits & 0.424 & -0.210 & 0.214 & 0.322 & 0.470 & 4.749\\
\hspace{1em}Number of emergent, non-preventable visits & 0.099 & -0.104 & 0.034 & 0.070 & 0.113 & 1.265\\
\hspace{1em}Number of emergent, preventable visits & -0.014 & -0.139 & -0.023 & -0.003 & 0.014 & 0.426\\
\hspace{1em}Number of primary care treatable visits & 0.201 & -0.084 & 0.101 & 0.146 & 0.217 & 2.053\\
\hspace{1em}Number of non-emergent visits & 0.144 & -0.015 & 0.083 & 0.115 & 0.165 & 1.210\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item Note: Estimates for quantiles of the ITE distribution using the Oregon Health Insurance Experiment data.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/Tables_final/tvarimp-all.tex <==
\begin{table}[t]

\caption{\label{tab:varimp.all}Variable importance scores}
\centering
\fontsize{9}{11}\selectfont
\makebox[\textwidth][c]{
\begin{threeparttable}
\begin{tabular}[t]{lr}
\toprule
Variable & Importance\\
\midrule
\addlinespace[0.3em]
\multicolumn{2}{c}{\textbf{Any visit}}\\
\hspace{1em}Pre-lottery SNAP benefit amount (\$) & 0.18\\
\hspace{1em}Age (years) & 0.18\\
\hspace{1em}Sum of total ED charges & 0.09\\
\hspace{1em}Number of emergent, non-preventable visits & 0.09\\
\hspace{1em}Number of primary care treatable visits & 0.08\\
\hspace{1em}Week of lottery sign up & 0.05\\
\hspace{1em}Number of non-emergent visits & 0.05\\
\hspace{1em}Female & 0.04\\
\hspace{1em}Number of emergent, preventable visits & 0.02\\
\hspace{1em}Number of visits (chronic conditions) & 0.01\\
\addlinespace[0.3em]
\multicolumn{2}{c}{\textbf{Any non-emergent visit}}\\
\hspace{1em}Sum of total ED charges & \vphantom{1} 0.13\\
\hspace{1em}Number of primary care treatable visits & 0.12\\
\hspace{1em}Number of outpatient visits & 0.12\\
\hspace{1em}Pre-lottery SNAP benefit amount (\$) & 0.12\\
\hspace{1em}Age (years) & 0.08\\
\hspace{1em}Number of non-emergent visits & \vphantom{1} 0.08\\
\hspace{1em}Number of emergent, non-preventable visits & 0.07\\
\hspace{1em}Number of inpatient visits & 0.04\\
\hspace{1em}Number of emergent, preventable visits & 0.04\\
\hspace{1em}Number of visits (chronic conditions) & 0.02\\
\addlinespace[0.3em]
\multicolumn{2}{c}{\textbf{Number of visits}}\\
\hspace{1em}Number of primary care treatable visits & 0.14\\
\hspace{1em}Sum of total ED charges & 0.13\\
\hspace{1em}Number of emergent, non-preventable visits & 0.10\\
\hspace{1em}Number of non-emergent visits & 0.08\\
\hspace{1em}Number of outpatient visits & 0.08\\
\hspace{1em}Number of overall visits & 0.08\\
\hspace{1em}Number of off-hours visits & \vphantom{1} 0.06\\
\hspace{1em}Number of emergent, preventable visits & 0.06\\
\hspace{1em}Pre-lottery SNAP benefit amount (\$) & 0.05\\
\hspace{1em}Age (years) & 0.04\\
\addlinespace[0.3em]
\multicolumn{2}{c}{\textbf{Number of non-emergent visits}}\\
\hspace{1em}Number of emergent, non-preventable visits & 0.16\\
\hspace{1em}Number of primary care treatable visits & 0.16\\
\hspace{1em}Sum of total ED charges & 0.12\\
\hspace{1em}Number of non-emergent visits & 0.09\\
\hspace{1em}Number of outpatient visits & 0.09\\
\hspace{1em}Number of off-hours visits & 0.06\\
\hspace{1em}Number of overall visits & 0.06\\
\hspace{1em}Number of emergent, preventable visits & 0.05\\
\hspace{1em}Pre-lottery SNAP benefit amount (\$) & 0.04\\
\hspace{1em}Number of inpatient visits & 0.03\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item Note: 
\end{tablenotes}
\end{threeparttable}
}
\end{table}


==> Tables/Tables_final/tvarimp-any.tex <==
\begin{table}[t]

\caption{\label{tab:varimp.any}Variable importance scores}
\centering
\fontsize{9}{11}\selectfont
\makebox[\textwidth][c]{
\begin{threeparttable}
\begin{tabular}[t]{lrlr}
\toprule
\multicolumn{2}{c}{Any visit} & \multicolumn{2}{c}{Any non-emergent visit} \\
\cmidrule(l{3pt}r{3pt}){1-2} \cmidrule(l{3pt}r{3pt}){3-4}
Variable & Importance & Variable & Importance\\
\midrule
Pre-lottery SNAP benefit amount (\$) & 0.18 & Sum of total ED charges & 0.13\\
Age (years) & 0.18 & Number of primary care treatable visits & 0.12\\
Sum of total ED charges & 0.09 & Number of outpatient visits & 0.12\\
Number of emergent, non-preventable visits & 0.09 & Pre-lottery SNAP benefit amount (\$) & 0.12\\
Number of primary care treatable visits & 0.08 & Age (years) & 0.08\\
Week of lottery sign up & 0.05 & Number of non-emergent visits & 0.08\\
Number of non-emergent visits & 0.05 & Number of emergent, non-preventable visits & 0.07\\
Female & 0.04 & Number of inpatient visits & 0.04\\
Number of emergent, preventable visits & 0.02 & Number of emergent, preventable visits & 0.04\\
Number of visits (chronic conditions) & 0.01 & Number of visits (chronic conditions) & 0.02\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item Note: 
\end{tablenotes}
\end{threeparttable}
}
\end{table}


==> Tables/Tables_final/tvarimp-ne.tex <==
\begin{table}[t]

\caption{\label{tab:varimp.ne}Variable importance scores}
\centering
\fontsize{9}{11}\selectfont
\makebox[\textwidth][c]{
\begin{threeparttable}
\begin{tabular}[t]{lrlr}
\toprule
\multicolumn{2}{c}{Any non-emergent visit} & \multicolumn{2}{c}{Number of nonemergent visits} \\
\cmidrule(l{3pt}r{3pt}){1-2} \cmidrule(l{3pt}r{3pt}){3-4}
Variable & Importance & Variable & Importance\\
\midrule
Sum of total ED charges & 0.13 & Number of emergent, non-preventable visits & 0.16\\
Number of primary care treatable visits & 0.12 & Number of primary care treatable visits & 0.16\\
Number of outpatient visits & 0.12 & Sum of total ED charges & 0.12\\
Pre-lottery SNAP benefit amount (\$) & 0.12 & Number of non-emergent visits & 0.09\\
Age (years) & 0.08 & Number of outpatient visits & 0.09\\
Number of non-emergent visits & 0.08 & Number of off-hours visits & 0.06\\
Number of emergent, non-preventable visits & 0.07 & Number of overall visits & 0.06\\
Number of inpatient visits & 0.04 & Number of emergent, preventable visits & 0.05\\
Number of emergent, preventable visits & 0.04 & Pre-lottery SNAP benefit amount (\$) & 0.04\\
Number of visits (chronic conditions) & 0.02 & Number of inpatient visits & 0.03\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item Note: 
\end{tablenotes}
\end{threeparttable}
}
\end{table}


==> Tables/Tables_final/tvarimp-num.tex <==
\begin{table}[t]

\caption{\label{tab:varimp.num}Variable importance scores}
\centering
\fontsize{9}{11}\selectfont
\makebox[\textwidth][c]{
\begin{threeparttable}
\begin{tabular}[t]{lrlr}
\toprule
\multicolumn{2}{c}{Number of visits} & \multicolumn{2}{c}{Number of nonemergent visits} \\
\cmidrule(l{3pt}r{3pt}){1-2} \cmidrule(l{3pt}r{3pt}){3-4}
Variable & Importance & Variable & Importance\\
\midrule
Number of primary care treatable visits & 0.14 & Number of emergent, non-preventable visits & 0.16\\
Sum of total ED charges & 0.13 & Number of primary care treatable visits & 0.16\\
Number of emergent, non-preventable visits & 0.10 & Sum of total ED charges & 0.12\\
Number of non-emergent visits & 0.08 & Number of non-emergent visits & 0.09\\
Number of outpatient visits & 0.08 & Number of outpatient visits & 0.09\\
Number of overall visits & 0.08 & Number of off-hours visits & 0.06\\
Number of off-hours visits & 0.06 & Number of overall visits & 0.06\\
Number of emergent, preventable visits & 0.06 & Number of emergent, preventable visits & 0.05\\
Pre-lottery SNAP benefit amount (\$) & 0.05 & Pre-lottery SNAP benefit amount (\$) & 0.04\\
Age (years) & 0.04 & Number of inpatient visits & 0.03\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item Note: 
\end{tablenotes}
\end{threeparttable}
}
\end{table}

